Frequency-Domain Identification of Discrete-Time Systems using Sum-of-Rational Optimization

We propose a computationally tractable method for the identification of stable canonical discrete-time rational transfer function models, using frequency domain data. The problem is formulated as a global non-convex optimization problem whose objective function is the sum of weighted squared residuals at each observed frequency datapoint. Stability is enforced using a polynomial matrix inequality constraint. The problem is solved globally by a moment-sum-of-squares hierarchy of semidefinite programs through a framework for sum-of-rational-functions optimization. Convergence of the moment-sum-of-squares program is guaranteed as the bound on the degree of the sum-of-squares polynomials approaches infinity. The performance of the proposed method is demonstrated using numerical simulation examples.

==> sections/acknowledgements.tex <==
\begin{ack}

The authors would like to thank Roland Toth, No\"{e}l Hallemans, and Mario Sznaier for discussions about sum-of-rational system identification.

% \urg{Optional acknowledgements.}
\end{ack}

==> sections/app_duality.tex <==

\section{Duality of Sum-of-Rational LPs}    % Each appendix must have a short title.
% \section{More Appendices}              % Sections and subsections are supported  
\label{app:strong_dual_lp}

This appendix will prove duality relations between \eqref{eq:rational_meas_sparse} $(p^*)$ and \eqref{eq:rational_cont_sparse} $(d^*)$. Notation and conventions will be used from Theorem 2.5 of \citep{tacchi2021moment}. Assumptions A1-A3 will be in place.


% This appendix proves strong duality between \eqref{eq:slice_upper_stokes} and \eqref{eq:slice_upper_meas_stokes}. The structure of the weak duality portion will follow the format of Appendix \ref{app:duality}.
\subsection{Weak Duality}
The optimization variables of \eqref{eq:rational_meas_sparse} and \eqref{eq:rational_cont_sparse} may be cast into terms $\bbmu$ and $\bell$ as
\begin{align}
  \bbmu &= (\mu, \{\nu_f\}_{f=1}^{N_f}), & \bell &= (\gamma, \{\zeta_f\}_{f=1}^{N_f})
  \label{eq:bell}
\end{align}

The measures $\bbmu$ are described by the spaces of 
\begin{align}    
    \mathcal{X} &= \mathcal{M}(\K)^{N_f+1} & 
    \mathcal{X}' &=  C(\K)^{N_f+1}, \\\label{eq:dual_spaces}
\intertext{possessing nonnegative subcones}
    \mathcal{X}_+ &= \mathcal{M}_+(\K)^{N_f+1}  &     \mathcal{X}'_+ &=  C_+(\K)^{N_f+1} \label{eq:dual_cones}.\\
\end{align}

The variable $\bell$ has the spaces 
\begin{align}
    \mathcal{Y} &= 0 \times ([\R[a, b]']^{N_f}), & \mathcal{Y}' &=\R \times \R[a, b]^{N_f},
\end{align}
where $\R[a, b]'$ is the dual space of polynomials (moment sequences). We use the convention $\mathcal{Y}_+ = \mathcal{Y}$ and $\mathcal{Y}_+' = \mathcal{Y}'$ due to the lack of moment-inequality constraints \citep{tacchi2021moment}.

The cost-vectors of \eqref{eq:rational_meas_sparse} and \eqref{eq:rational_cont_sparse} respectively are
% \begin{subequations}
% \label{eq:cost_constraint}
    \begin{align}        
        \mathbf{c} &= [0, \ \{p_f(a,b)\}_{f=1}^{N_f}],  & 
        \mathbf{b} &= [1, \ \{0\}_{f=1}^{N_f}],
        \intertext{forming the variate pairings}
        \inp{\mathbf{c}}{\bbmu} &= \textstyle \sum_{f=1}^{N_f} \inp{p_f}{\nu_f} & \inp{\mathbf{b}}{\bell} &= \gamma.
    \end{align}
% \end{subequations}


Let us express constraint \eqref{eq:rational_meas_sparse_mult} in the shorthand form of \begin{equation}
    \forall f \in 1..N_f: \qquad q_f^\dagger \nu_f = \mu,
\end{equation}
enumerating over all test monomials $a^\alpha b^\beta$.

We can define an affine operator $\mathcal{A}: \mathcal{X} \rightarrow Y'$ and adjoint  $\mathcal{A}^\dagger: Y \rightarrow \mathcal{X}'$ acting on $(\bbmu, \bell)$ as
\begin{align}
    \mathcal{A}(\bbmu) &= [\inp{1}{\mu}, \forall f \in 1..N_f: \  q_f^\dagger \nu_f - \mu] \\
    \mathcal{A}^*(\bell) &= [\textstyle \sum_{f=1}^{N_f} \zeta_f - \gamma, \ \forall f \in 1..N_f: \  p_f - \zeta_f q_f ].\nonumber
\end{align}

Problems \eqref{eq:rational_meas_sparse} and \eqref{eq:rational_cont_sparse} can be placed in standard conic form as 
\begin{align}
        p^* = &\inf_{\boldsymbol{\ell} \in \mathcal{Y}'_+} \inp{\boldsymbol{\ell}}{\mathbf{b}}
    & &\A'(\boldsymbol{\ell}) - \mathbf{c} \in \mathcal{X}_+, \label{eq:slice_cont_std} \\
        d^* =& \sup_{\boldsymbol{\mu} \in \mathcal{X}_+} \inp{\mathbf{c}}{\boldsymbol{\mu}} & & \mathbf{b} - \A(\boldsymbol{\mu}) \in \mathcal{Y}_+, \label{eq:slice_meas_std}
\end{align}
thus ensuring weak duality for $\K_0$ and $\K_s$ \citep{barvinok2002convex}.

\subsection{Strong Duality}

This subsection will prove strong duality over $\K_s$. Strong duality between \eqref{eq:rational_meas_sparse} and \eqref{eq:rational_cont_sparse} will occur if the following sufficient conditions are obeyed (Theorem 2.6 of \citep{tacchi2021moment}):
\begin{itemize}
    \item[R1] Every feasible measure $\bbmu \in \mathcal{X}_+: \mathcal{A}(\bbmu) \in \mathcal{Y}_+$ is finite.
    \item[R2] Such a finite feasible measure exists.
    \item[R3] All entries of $(\mathcal{A}, \mathbf{b}, \mathbf{c})$ are continuous in $(a, b)$.
\end{itemize}
Satisfaction of R1-R3 will additionally impose that the infimum of \eqref{eq:rational_meas_sparse} and supremum of \eqref{eq:rational_cont_sparse} are attained (over $\K_s$).

Finiteness (boundedness) of measures in R1 will be proven by noting that all measures in $\bbmu$ have compact support and finite mass. The measure $\mu$ is a probability measure (mass 1) by \eqref{eq:rational_meas_sparse_obj}. Because each $q_f$ is positive over $\K_s$ (Lemma \ref{lem:q_pos_stab}) and $q_f$ is continuous over $\K_s$ (a polynomial), it holds that $1/q_f(a)$ is continuous, positive, and bounded over $\K_s$. By the Stone-Weierstrass theorem \citep{stone1948generalized}, there also exists a sequence of polynomials $\psi_k \in \R[a]$ that converges uniformly to $1/q_f(a)$ over $\K_s$. The linearity of constraint 
\eqref{eq:rational_meas_sparse_mult} will produce 
the relations
\begin{align}
     & \forall (\alpha, \beta) \in \N^{2n}, \ f \in 1..N_f, \  k \in \N: \nonumber \\
    & \qquad \inp{\psi_k(a) q_f(a)}{\nu_f (a, b)} = \inp{\psi_k(a)}{\mu(a, b)}. \label{eq:rational_meas_sparse_psi}
    \intertext{Weak convergence as $k \rightarrow \infty$ will form}
    & \qquad \inp{1}{\nu_f} = \inp{1/q_f(a)}{\mu}.
\end{align}
As such, all measures in $\bbmu$ are finite, and R1 is satisfied.

% \urg{Check if weak convergence is correct.}

The construction from the proof of Theorem \ref{thm:meas_lower_bound} will produce a feasible measure $\bbmu$ from a reference system $(a', b') \in \K_s$, fulfilling R2.

For R3, we note that $p_f$ in $\mathbf{c}$ are polynomial functions (continuous), and $b$ is a constant vector. Furthermore, the operator $\mathcal{A}$ entails multiplication by the continuous polynomials $q_f$ when forming constraint \eqref{eq:rational_meas_sparse_mult}.

Because requirements R1-R3 are all met, strong duality and optima attainment occur between \eqref{eq:rational_meas_sparse} and \eqref{eq:rational_cont_sparse}.

\subsection{Failure of Strong Duality without Stability}

Lemma \ref{lem:nonneg_unstab} states that each $q_f(a)$ is nonnegative over $\K_0$. The proof of Theorem \ref{thm:meas_lower_bound} notes that this nonnegativity could lead to cases (roots at sample frequencies $e^{j \omega_f}$) where the moments of $\nu_f$ are undefined in terms of $\mu$. The mass of feasible $\nu_f$ could therefore be unbounded,  violating R1 and thus failing strong duality. While strong duality over $\K_0$ may hold in specific problem instances, it cannot be guaranteed in general.

==> sections/app_fractional.tex <==
\section{Stability Constraints for Fractional-Order Systems}
\label{app:fractional}

% \urg{Fill this in}

This appendix will analyze conditions for stabilization of a single-input single-output commensurate fractional order linear system.



\urg{Matignon stability}



==> sections/extensions.tex <==
\section{Extensions}

\label{sec:extensions}

The sum-of-rational global optimization method  in \eqref{eq:gain_base} for system identification can be extended in several directions. All of these proposed extensions may be combined if desired.

% \subsection{Frequency Weighting}\label{sec:freq_weighting}

% A weighting function $W: \C \rightarrow \C$ can be introduced to encourage fidelity at specific frequencies. Letting $W_f = W(e^{j \omega_f})$ be the weight evaluated at frequency point $f$, a weighted version of the problem in \eqref{eq:gain_base} is 
% \begin{align}
%     P^* = \textstyle \inf_{a, b} \sum_{f=1}^{N_f} \abs{W_f(G_f - G(e^{j \omega_f}))}^2. \label{eq:gain_weighted}
% \end{align}

% The weighted numerators $p^W_f(a, b)$ modified from \eqref{eq:poly_base_num} in the frequency-weighted case are
% \begin{align}
% p_f^W(a, b) &= \abs{W_f G_f(1 + A(e^{-j \omega_f})) - W_f B(e^{-j \omega_f})}^2.
% \end{align}

\subsection{Minimax Estimation}
% \urg{Not sure what this one will be}
{\color{blue} The MSE objective can be justified using statistical reasoning. Can the min-max approach suggested here be motivated somehow ? What kind of estimator of (a,b) do we get here?}
\medskip

Problem \eqref{eq:gain_base} minimizes the \ac{MSE} of the error terms $\norm{\eta}_2^2.$ It is also possible to minimize the maximum error at any frequency point:
\begin{align}
    P^*_\infty =  \inf_{a, b} \max_{f \in 1..N_f} \abs{W_f\left(G_f - G(e^{j \omega_f}) \right)}^2. \label{eq:gain_inf}
\end{align}
A measure \ac{LP} for \eqref{eq:gain_inf} can be posed by introducing a new variable $\tau \in \R$ to upper-bound the magnitude-squared error $\abs{\eta_f}^2$ at each datapoint:

\begin{subequations}
\label{eq:rational_meas_sparse_inf}
\begin{align}
    p^*_\infty = &\textstyle  \inf_{\tau \in \R} \quad \tau \\
    & \inp{1}{\mu} = 1 \\
    & \forall (\alpha, \beta) \in \N^{2n}, f \in 1..N_f: \nonumber \\
    & \qquad \inp{a^\alpha b^\beta q_f(a)}{\nu_f (a, b)} = \inp{a^\alpha b^\beta }{\mu(a, b)} \label{eq:rational_meas_sparse_inf_mult}\\
    & \forall f \in 1..N_f: \quad \tau \geq \inp{p_f(a, b)}{\nu_f(a, b)} \\
    & \mu \in \Mp{\K} \label{eq:rational_meas_sparse_inf_mu}\\
    & \forall f \in 1..N_f: \ \nu_f \in \Mp{\K}.
\end{align}
\end{subequations}



==> sections/modified_transfer_functions.tex <==
\section{Other Sum-of-Rational Models}

\label{sec:other_rational}
Problem \eqref{eq:gain_base} sought to identify a discrete-time dynamical system based on Bode-plot data. This subsection details the use of the proposed method for other models and experimental configurations.

\subsection{Continuous-Time Systems}
The data in $\dc$ can also be used to identify a continuous-time dynamical system (under bandlimited data) with the objective of 
\begin{align}
    P^*_c =  \inf_{(a, b)} \sum_{f=1}^{N_f} \abs{G_f - G(j \omega_f)}^2. \label{eq:gain_base_cont}
\end{align}

The numerator and denominator polynomials in \eqref{eq:poly_base} would be modified accordingly with arguments of $-j\omega_f$ rather than $e^{-j \omega}$.

Let $a_1 = [1; a]$ and $\tilde{a}_1$ be the coefficients of $1+A(z)$ and $1+A(-z)$ respectively. A matrix $Q \in \psd^n$ may be constructed from \cite{henrion2003ellipsoidal} by 
% Let $a_1 = [1; a]$ and $\tilde{a}_1 = [$
% The Hermite matrix for a continuous time system is the unique solution to
\begin{align}
    Q = a_1 a_1^T - \tilde{a}_1 \tilde{a}_1,
\end{align}
resulting in the Hurwitz continuous-time stability relation (roots on stable left-half plane) of
\begin{equation}
\label{eq:stable_hermite}
    0 = \begin{bmatrix}
        0_{n \times 1} & H \\ 0 & 0_{1 \times n} 
    \end{bmatrix}  + \begin{bmatrix}
         0_{1 \times n}  & 0 \\ H &  0_{n \times 1}
    \end{bmatrix}.
\end{equation}
% The unique solution to \eqref{eq:stable_hermite} may be discovered through the following dynamic-programming-type iteration:
% \begin{align}
%     \forall j\in 2..n_a-1, i\in 1..n_a-1
%     H_{i,j} = Q_{i+1, j} - H_{i+1, j-1}
% \end{align}
% \urg{Write the Hermite Matrix for continuous-time systems.
% Is it
% \begin{equation}
%     0 = \begin{bmatrix}
%         0_{n \times 1} & H \\ 0 & 0_{1 \times n} 
%     \end{bmatrix}  + \begin{bmatrix}
%          0_{1 \times n}  & 0 \\ H &  0_{n \times 1}
%     \end{bmatrix}
% \end{equation}

% }

\subsection{Closed-Loop System Identification}

The Bode-plot data in $\dc$ for \eqref{eq:gain_base} was collected in open-loop. This extension involves the case where the unknown plant $G(z) = B(z^{-1})/(1+A(z^{-1}))$ is connected in feedback with a known dynamic compensator $C(z) = \tilde{B}(z^{-1})/(1+\tilde{A}(z^{-1})).$ The closed-loop transfer function in this case is given as

\begin{align}
G^{cl}(z) &= 
    \frac{B^{cl}(z^{-1})}{1+A^{cl}(z^{-1})}= \frac{G(z^{-1})}{1 + G(z^{-1}) C(z^{-1})} \label{eq:closed_loop} \\ 
    & = \frac{B(z^{-1}) (1+\tilde{A}(z^{-1}))}{(1+A(z^{-1}))(1+ \tilde{A}(z^{-1})) + B(z^{-1}) \tilde{B}(z^{-1})} \nonumber 
    \end{align}

The closed-loop optimization problem becomes
\begin{align}
    P^*_{cl} =  \inf_{(a, b)} \sum_{f=1}^{N_f} \abs{G_f^{cl} - G^{cl}(e^{j \omega_f})}^2. \label{eq:gain_closed_loop}
\end{align}

The following functions may be defined:
\begin{subequations}
\label{eq:poly_closed}
\begin{align}
  \!\!\! \!\!\! D_f^{cl}(a, b) &= (1+A(e^{-j \omega_f}))(1+ \tilde{A}(e^{-j \omega_f}))  \nonumber \\
    & \qquad + B(e^{-j \omega_f}) \tilde{B}(e^{-j \omega_f}) \\    
  \!\!\! \!\!\! p_f^{cl}(a, b) &= \abs{G_f D_f(a, b) - B(e^{-j \omega_f})(1 + \tilde{A}(e^{-j \omega_f}))}^2 \label{eq:poly_base_num_closed}\\
   \!\!\!\!\!\! q_f^{cl}(a) &= \abs{D_f(a, b)}^2,
\end{align}
\end{subequations}
% may be expressed as a sum of rational functions
% after requisite algebraic manipulations into
    % We can express \eqref{eq:closed_loop} at each frequency datapoint $f$ as a rational function of the plant parameters $(a, b)$ after requisite algebraic manipulations
    % \begin{align}
    %     G^{cl}_f = p^{cl}_f(a, b)/q^{cl}_f(a, b).
    % \end{align}
    % Problem \eqref{eq:gain_base} can therefore be expressed in the closed-loop case as 
to create the sum-of-rational-functions form for \eqref{eq:gain_closed_loop} as    
    \begin{align}
\label{eq:rational_closed}
    P^*_{cl} = \inf_{(a, b)} \textstyle \sum_{f=1}^{N_f} \frac{p_f^{cl}(a, b)}{q_f^{cl}(a, b)}.
\end{align} 

Note that the denominator polynomial $q_f^{cl}$ in \eqref{eq:rational_closed} depends on $b$, due to the feedback with $C(z)$ in \eqref{eq:closed_loop}. The moment-\ac{SOS} \ac{LMI} derived from  a degree-$d$ truncation of \eqref{eq:rational_closed} will therefore not generally possess term sparsity \citep{wang2021tssos}.

If it is assumed that the closed-loop system $G^{cl}(z)$ is stable, then the Hermite stability constraint in $\mathcal{S}$ must be posed over the non-constant-coefficient vector of the closed-loop denominator in \eqref{eq:closed_loop} ($1+G(z^{-1}) C(z^{-1})$).



==> sections/outliers.tex <==
\section{Outlier-Robust System Identification}
\label{sec:outlier}
We can extend the system identification methods towards identification and rejection of outliers contaminating $\dc$. 

\subsection{Outlier-Robust Setting}

Assume that we have a budget of $N_{\textrm{out}}$ outliers in the frequency-domain data. We can define a binary variable $s_f \in \{0, 1\}$ for each datapoint and pose the following outlier-rejection problem:

\begin{align}
\label{eq:rational_outlier}
    P^* =&  \quad \inf \textstyle \sum_{f=1}^{N_f} (1-s_f) \abs{W_f\left(G_f - G\left(e^{j \omega_f}; (a,b)\right)\right)}^2  \nonumber \\
    & \forall f \in 1..N_f: \quad s_f \in \{0, 1\} \nonumber \\
    & \textstyle \sum_{k=1}^{N_f} s_f \leq N_{\textrm{out}}. 
\end{align}

The binary variable $s_f$ is $0$ if frequency point $f$ is an inlier, and $s_f=1$ if $f$ is an outlier.

% \subsection{Sparse Sum-of-Rational Program Background}

\subsection{Sparse Outlier Measure Program}

We can define measures $\mu_f(a, b, s_f)$ and $\nu_f(a, b, s_f)$ for each frequency point $f \in \{1, \dots, N_f\}$. The support of each measure is $\Mp{\K \times \{0, 1\}}$, in which the per-frequency binary support can be represented by the equality constraint $s_f^2 = s_f$.

A measure program for \eqref{eq:rational_outlier} will have the form of

\begin{subequations}
\label{eq:rational_meas_sparse_outlier}
\begin{align}
    p^*_{\textrm{out}} = \inf &\sum_{f=1}^{N_f} \inp{(1-s_f)p_f(a, b)}{\nu_f} \\
    & \inp{1}{\mu_1} = 1 \\
    & \textstyle \sum_{f=1}^{N_f} \inp{s_f}{\mu_f} \leq N_{\textrm{out}} \\
    & \forall (\alpha, \beta) \in \N^{2n}, f \in 1..N_f: \nonumber \\
    & \qquad \inp{a^\alpha b^\beta q_f}{\nu_f} = \inp{a^\alpha b^\beta}{\mu_f} 
    \label{eq:rational_meas_sparse_outlier_mult}\\
    & \forall (\alpha, \beta) \in \N^{2n-1}, f \in 1..N_f: \nonumber \\
    & \qquad \inp{a^\alpha b^\beta s_f q_f}{\nu_f} = \inp{a^\alpha b^\beta s_f}{\mu_f} 
    \label{eq:rational_meas_sparse_outlier_mult_bin}\\
    & \forall (\alpha, \beta) \in \N^{2n}, f \in 1..N_f-1: \nonumber \\
    & \qquad \inp{a^\alpha b^\beta}{\mu_f (a, b, s_f)} \\ \nonumber
    &\qquad\qquad  = \inp{a^\alpha b^\beta}{\mu_{f+1}(a, b, s_{f+1})} 
    \label{eq:rational_meas_sparse_outlier_csp}\\  
    & \forall f \in 1..N_f: \ \mu_f, \ \nu_f \in \Mp{\K \times \{0, 1\}}.
\end{align}
\end{subequations}

Constraints \eqref{eq:rational_meas_sparse_outlier_mult} and \eqref{eq:rational_meas_sparse_outlier_mult_bin} ensure that $\nu_f$ has a density of $1/D_f$ w.r.t. $\mu_f$ for each $f$. Constraint \eqref{eq:rational_meas_sparse_outlier_csp} is a correlative-sparsity constraint, ensuring that the $(a, b)$-marginal of each $\mu_f$ are in alignment (equal). Equivalence and convergence of \eqref{eq:rational_outlier} to  \eqref{eq:rational_meas_sparse_outlier} is provided by Theorem 3.2 of \cite{bugarin2016minimizing} under the stability constraint $(\K = \K_s)$.


==> sections/stable_system.tex <==
\section{Schur-Stable System Identification}

A plant $(a^*, b^*)$ recovered from a globally-optimal  solution of \eqref{eq:sum_of_rational_mom_abscont_sysid} is not guaranteed to be Schur stable.

% Schur stability $A(z^{-1})$

% Schur stability (or more generally the placement of the roots of $A(z^{-1})$ in an \ac{LMI} region) can be enforced through the use of a Hermite-Matrix Positive Definite condition explained in \cite{henrion2003ellipsoidal, henrion2011inner}.
% Following the procedure of \cite{henrion2011inner}, the matrices $\Theta(a)$ and $\tilde{\Theta}(a)$ can be defined as
% \begin{align}
%     \Theta(a) = \begin{bmatrix}
%         1 & a_1 & a_2 & \hdots\\
%         0 & 1 & a_1 & \hdots \\
%         0 & 0 & 1 & \hdots \\
%         \vdots & \vdots & \vdots & \ddots
%     \end{bmatrix} &  \tilde{\Theta}(a) = \begin{bmatrix}
%         a_n & a_{n-1} & a_{n-2} & \hdots\\
%         0 & a_n & a_{n-1} & \hdots \\
%         0 & 0 & a_n & \hdots \\
%         \vdots & \vdots & \vdots & \ddots
%     \end{bmatrix},
%     \end{align}
% \begin{align}
%     \intertext{to form the symmetric-matrix-valued polynomial}
%     \Xi(a) = \Theta(a)^T \Theta(a) - \tilde{\Theta}(a)^T \tilde{\Theta}(a).
% \end{align}

The class of polynomials $z^n(1+A(z^{-1}))$ \urg{correct exponents?} with roots $\abs{z}<1$ is represented by a \ac{PMI} of \cite{henrion2011inner}
\begin{align}
    a \in \R^n: \qquad  \Xi(a) \succ 0. \label{eq:stable_pmi}
\end{align}

The identified plant $(a, b)$  from \eqref{eq:sum_of_rational_mom_abscont_sysid} will be Schur stable after adding the \ac{PMI} \eqref{eq:stable_pmi} into the constraint set $\K$. The localizing matrix constraint \eqref{eq:stable_pmi} has an expression of
\begin{align}
    &\forall f(a, b) \in (\R[a, b])^{n}: \\
    & \qquad L_{y}(f(a, b)^T \Xi(a) f(a, b)) > 0,
\end{align}
which can be represented by a strict \ac{LMI} in $y$ of maximal \ac{PSD} size $n \binom{n+d}{d}$ (or for $y^f$ of size $n \binom{n+d+1}{d+1}$) \citep{scherer2006matrix}.

\urg{How does the Hermite matrix in $\Xi$ look  if we want to be in the nonstrict region $\norm{z} \leq \rho$? The considered \ac{BSA} sets are all closed.}

% We can also impose that the recovered  polynomial $A(z^{-1})$ is stable, or more appropriately has all of its roots located in a given open ellipse.

% This support condition in $a$ may be imposed through the use of a Hermite-Matrix Positive Definite condition explained in \cite{henrion2003ellipsoidal, henrion2011inner}. We can then use a Scherer Psatz of nonnegativity \cite{scherer2006matrix} to ensure that the rational function is supported over this Polynomial Matrix Inequality.

% The Hermite criterion of 

We can add this positive-definite expression in \eqref{eq:stable_pmi} into the $\mu$ support constraint in \eqref{eq:rational_meas_sparse_mu}.


==> sections_extended/abstract_extended.tex <==
\begin{abstract}
\label{sec:abstract}
This work proposes a computationally tractable method for the identification of canonical rational transfer function models, using a finite set of input-output measurements. The problem is formulated in frequency-domain as a global optimization problem whose cost function is the sum of weighted squared residuals at each observed frequency datapoint. It is solved by the moment-sum-of-squares hierarchy of semidefinite programs, through a framework for sum-of-rational-functions optimization from Bugarin, Henrion, Lasserre 2016. The generated program contains decomposable term sparsity \cite{wang2021tssos} which can be exploited for further computational complexity reductions. Convergence of the moment-sum-of-squares program is guaranteed as the bound on the degree of the sum-of-squares polynomials approaches infinity. We discuss extensions of this rational-program method for identification of stable systems, and closed-loop identification. 
% \urg{figure out which extensions we want to include}

% \urg{Abstract goes here}

% \urg{Let's use this as a working document/Arxiv version. We can cut down to 6 pages (for conference) later.}

\end{abstract}

==> sections_extended/acknowledgements.tex <==
\section*{Acknowledgements}

The authors would like to thank Roland Toth, No\"{e}l Hallemans, and Mario Sznaier for discussions about sum-of-rational system identification.

% \urg{Optional acknowledgements.}


==> sections_extended/conclusion.tex <==
\section{Conclusion}

\label{sec:conclusion}

We proposed a method of estimating canonical rational transfer functions based on the global minimization of a frequency-response weighted 2-norm objective. The original non-convex problem in \eqref{eq:gain_base} was converted to an equivalent linear program in measures by using a sum-of-rational formulation. Certifiable global optima can be obtained through moment-\ac{SOS}-based truncations of the linear program in measures. This linear program in measures obtains strong duality with a linear program in functions under compactness and finiteness assumptions. The proposed method can be extended to cases including continuous-time systems, closed-loop  identification and oultlier-corrupted settings.

% \urg{some other sentence reflecting the contents of this paper.}
% This flexible method was extended towards other transfer functions, weightings, and stable system identification.

% \urg{Conclude the paper. Summarize the problem and important findings. Add some extensions and future work.}

% The extended version of this paper at \cite{abdalmoaty2023rationalsysid} includes further discussions about strong duality, identification of continuous-time systems,  closed-loop identification, and identification of outlier-corrupted data.
% (using the sparse sum-of-rational framework of Theorem 3.2 of \cite{bugarin2016minimizing}).
% Future work includes the investigation of statistical properties (e.g., bias and variance) for the minimal \ac{MSE} estimators in \eqref{eq:gain_base}, \eqref{eq:gain_closed_loop}. 
Future work includes %derivations of statistical properties of estimators, 
the addition of regularization terms in order to prevent overfitting the noise process, and a homogenized formulation to reduce the conservatism of Assumption \ref{assum1}. Other work includes improvement of the \ac{SDP}'s numerical conditioning, especially for cases where the poles are close to the boundary of the unit disk.
% what will the arxiv version have that this work does not?,


==> sections_extended/function_lp.tex <==
\subsection{Function Linear Program}

The dual of \eqref{eq:rational_meas_sparse} may be derived after the introduction of dual variables $\lambda \in \R$ and $\forall f: \zeta_f \in \R[a, b]$. The dual program for \eqref{eq:rational_meas_sparse} is
\begin{subequations}
\label{eq:rational_cont_sparse}
    \begin{align}
        d^* = & \sup \lambda \\
        & \forall  (a, b) \in \K: \\
        & \qquad \textstyle \left(\sum_{f=1}^{N_f} \zeta_f(a, b) \right) - \gamma \geq 0 & & \label{eq:rational_cont_sparse_q}\\
        & \forall f \in \{1, \ldots, N_f\}, \forall (a, b) \in \K: \\
        & \qquad  p_f(a, b) - \zeta_f(a, b) q_f(a) \geq 0 & &  \label{eq:rational_cont_sparse_qf} \\
        & \lambda \in \R \\
        & \forall f \in \{1, \ldots, N_f\}: \quad \zeta_f(a, b) \in \R[a, b].
    \end{align}
\end{subequations}
\smallskip

\begin{thm}
\label{thm:strong_dual}
    Weak duality $(p^* \geq d^*)$ holds between \eqref{eq:rational_meas_sparse} and \eqref{eq:rational_cont_sparse} under A1-A3 over $\K_0$, and strong duality $(p^* = \ell^*)$ occurs over $\K_s$.
\end{thm}
\begin{pf}
    See Appendix \ref{app:strong_dual_lp}.
\end{pf}

Strong duality ensures that a control practitioner who implements an \ac{SOS}-truncation of \eqref{eq:rational_cont_sparse} (such as in \citep{wang2021tssos}) will receive the same solution as moment truncations to \eqref{eq:sum_of_rational_meas}.

% \urg{I can write a bit about the dual program and strong duality if we would like. TSSOS uses the dual (SOS) form.}



==> sections_extended/introduction.tex <==
\section{Introduction}
\label{sec:introduction}


Fitting parametric \ac{LTI} models to noisy frequency domain data is a classical problem in system identification \citep{pintelon2012, ljung1999}. Many methods and algorithms based on stochastic as well as deterministic frameworks have been developed and used. In particular, the \ac{ML} method, and  \acp{PEM} are frequently used due to their optimal asymptotic  statistical properties; see \cite[Ch.~8 \& 9]{ljung1999} and \cite[Ch. 9.11]{pintelon2012}. They define estimators as  solutions to optimization problems; however, for a large class of models, their implementation is complicated by the fact that the resulting optimization problems are highly non-convex.  Solutions of \acp{PEM}/\ac{ML} are usually obtained by local numerical optimization algorithms \cite[Ch.~10]{ljung1999}, introducing the vulnerability of terminating at a local minimum without a guarantee of global optimally.

The goal of this paper is to perform parametric identification of rational \ac{LTI} systems through global optimization of a \ac{MSE} objective. For the example of a strictly proper discrete-time SISO system with a known fixed order $n$ parameterized by $(a, b) \in \R^n \times \R^n$,  the model is given in terms of a transfer function 
% Assume that our unknown strictly proper system with fixed order $n$ is 
\begin{align} \label{eq:transfer_function}
    G(z; (a,b)) = \frac{B(z^{-1})}{1+A(z^{-1})} = \frac{\sum_{k=1}^{n} b_k z^{-k}}{1 + \sum_{k=1}^n a_k z^{-k}}
\end{align}
where $z$ is the complex variable of the $\mathcal{Z}$-transform. 
The problem is formulated in frequency-domain using a sequence of 
$N_f$ corrupted Bode-plot data $G_f$ at frequencies $\omega_f$, forming the data set $\dc =\{(\omega_f, G_f)\}_{f=1}^{N_f}$ with frequency weights $W = \{W_f\}_{f=1}^{N_f}$ The data in $\dc$ is collected under the following observation process with residual $\eta_f$:
\begin{align}
    G_f = G_\circ(e^{j \omega_f}) + \eta_f. \label{eq:gain_datas}
\end{align}
where $G_\circ(e^{j \omega_f}) = G(e^{j \omega_f}; (a_\circ, b_\circ))$ denotes the true underlying system. When $G_\circ$ is replaced with $G\left(e^{j \omega_f}; (a,b)\right)$ the following weighted 2-norm of the residuals vector $\eta(a,b)$ is obtained
\begin{equation}
\begin{aligned}
    \mathcal{J}_\dc (a, b) &= \textstyle \norm{W \odot \eta(a, b)}_2^2 \\
    &= \textstyle \sum_{f=1}^{N_f}  \abs{W_f\left(G_f - G\left(e^{j \omega_f}; (a,b)\right)\right)}^2. \label{eq:mse_plant}
\end{aligned}
\end{equation}
Our goal is to identify a plant $(a^*, b^*)$ that infimizes this norm: 
\begin{align}
    P^* =  \inf_{a, b} \mathcal{J}_\dc (a, b). \label{eq:gain_base}
\end{align}



% Possible modifications of the problem in \eqref{eq:gain_base} can include continuous-time data ($\eta_f = G_f - G(j \omega_f)$), frequency-weighted least square error objectives, input-output observations in Fourier space ($\eta_f = Y_f - G(e^{j \omega}) U_f$).
The gain-\ac{MSE}-minimizing problem in \eqref{eq:gain_base} also appears in \cite{adcock1987curve} and in Equation (7.150) of \citep{ljung1999}.
Problem \eqref{eq:gain_base} is a nonconvex in the optimization variables $(a, b)$. The objective function can be cast as a sum of rational functions (sum of ratios) problem \cite{schaible1994fractional, freund2001solving}. 
Our work focuses on global optimization of \eqref{eq:gain_base} through the measure \ac{LP}-based sum-of-ratios framework introduced by \cite{bugarin2016minimizing}. The method in \citep{bugarin2016minimizing} uses the moment-\ac{SOS} \citep{lasserre2009moments} hierarchy of \acp{SDP} in order to obtain a nondecreasing sequence of lower bounds to $P^*$. Recovery of  global optimizers $(a^*, b^*)$ will occur if the \ac{PSD} solution matrices of the satisfy a rank condition \citep{curto1996solution, henrion2005detecting}.







% \urg{Introduction goes here. }

% \urg{

% % Literature review here.

% System identification, frequency domain methods. Why does our method matter?

% % Polynomial optimization, Rational optimization.

% % What we are proposing. How are we tying it all together?

% }

\subsection{Motivation}
The data set $\dc$ can be obtained via time-domain or frequency-domain experiments. In time-domain experiments, an excitation input signal is applied to the plant, and $N_f$ samples of the input and output signals are recorded. These are then transformed to the frequency domain using the discrete Fourier transform, and may then be used to obtain a non-parametric estimate $G_f$, using, e.g., an empirical transfer function estimator \citep[Ch. 6.3]{ljung1999}. In frequency-domain experiments, a single  sinusoidal excitation is applied to the plant, and the input-output spectra of the steady-state response are measured at the excited frequency. This process is repeated at $N_f$ different frequencies \citep[Ch. 6.2]{ljung1999}, giving rise to $\dc$.  

Since the discrete Fourier transform is unitary, there is an equivalence between time-domain and frequency-domain identification (see, e.g., \cite{aguero2010} for the case of \ac{ML} identification).  However, depending on the experimental setup and the used models, one domain may offer a significant computational advantage over the other. In this work, we exploit a computational advantage  offered in the frequency-domain: the residuals norm in \eqref{eq:gain_base} is decoupled over $N_f$ frequencies. This allows us to  reformulate the identification problem as an infinite-dimensional \ac{LP} over multiple measures, without introducing additional optimization variables in the original problem. It also allows for several straightforward extensions as explained later in the paper.

% Notice that the model in \eqref{eq:gain_datas} can be seen as a special case where the input $U_f = 1$ and the output $Y_f = G_f$. 

The model in \eqref{eq:gain_datas} abstracts out the uniformly weighted case ($W_f=1$ can be interpreted as $U_f = 1$ and the output $Y_f = G_f$) as well as the input-output case ($W_f = U_f$, $W_f G_f = Y_f$).
The estimator $\dc \mapsto (a^\ast, b^\ast)$ is then an output error estimator, that minimizes the difference between the observed output and the modelled output; namely, $Y_f - G(e^{j \omega_f}; (a,b)) U_f$. It is well-known that, in a stochastic framework assuming (asymptotically) zero mean mixing residuals, such an estimator is strongly consistent and asymptotically normal. Statistical efficiency is obtained for Gaussian residuals using inverse-variance weighting of the objective function (for details, see \citep[Ch. 8 \& 9]{ljung1999}). Similar properties can also be shown using a deterministic framework \citep{ljung1985}. 


\begin{comment}
{\color{blue}This part is not complete yet, I will work on it a bit later today or early next week. We need to assume something about $\eta$ to establish some properties of the obtained estimator; as for example what happens when $N \to \infty$ }
{\color{gray} 



Assuming a quasi-stationary residual, and using the definition of the inverse Fourier transform, 
\[
\lim_{N\to\infty} \frac{1}{N} \sum_{t=1}^{N} \mathbb{E}\; \eta_t^2 = R_\eta(0) = \frac{1}{2\pi} \int_{_\pi}^\pi
 \Phi_\eta(\omega) \; d\omega\]
where the spectrum of $\eta$ is
\[
 \Phi_\eta(\omega) \!=\!\!\! \sum_{\tau = - \infty}^\infty \!\!\!\! R_\eta(\tau) e^{-i\tau\omega}, \quad R_\eta(\tau) \!=\!\!\! \lim_{N\to\infty} \frac{1}{N} \sum_{t=1}^{N} \mathbb{E}\; \eta_t \eta_{t- \tau}. 
\]
From \eqref{eq:gain_datas}, 
\[
\begin{aligned}
\eta_f(a,b) &= G_f - G(e^{j \omega_f}; (a,b))\\
&= G_\circ(e^{j\omega_f}) - G(e^{j \omega_f}; (a,b)) + \eta_f(a_\circ, b_\circ)
\end{aligned}
\]

}

\end{comment}

\subsection{Contributions}
Earlier works that use the moment-\ac{SOS} hierarchy for parametric identification in time-domain are \citep{Rodrigues2019,Rodrigues2020}. These approaches are based on introducing the time-domain residuals as optimization variables, leading to sparse polynomial optimization problems. 
The closest prior work to our method is in \citep[Ch. 7]{vuillemin2014frequency}, in which model reduction of an \ac{LTI} system proceeds through a sum-of-ratios function optimization problem by minimizing the \ac{MSE} over a pole-residue partial fraction expansion. 

==> sections_extended/modified_transfer_functions.tex <==
\section{Other Sum-of-Rational Models}

\label{sec:other_rational}
Problem \eqref{eq:gain_base} sought to identify a discrete-time dynamical system based on Bode-plot data. This subsection details how other experimental 

\subsection{Continuous-Time Systems}
The data in $\dc$ can also be used to identify a continuous-time dynamical system (under bandlimited data) with the objective of 
\begin{align}
    P^*_c = \textstyle \inf_{a, b} \sum_{f=1}^{N_f} \abs{G_f - G(j \omega_f)}^2. \label{eq:gain_base_cont}
\end{align}

The numerator and denominator polynomials in \eqref{eq:poly_base} would be modified accordingly with arguments of $-j\omega_f$ rather than $e^{-j \omega}$.

Let $a_1 = [1; a]$ and $\tilde{a}_1$ be the coefficients of $1+A(z)$ and $1+A(-z)$ respectively. A matrix $Q \in \psd^n$ may be constructed from \cite{henrion2003ellipsoidal} by 
% Let $a_1 = [1; a]$ and $\tilde{a}_1 = [$
% The Hermite matrix for a continuous time system is the unique solution to
\begin{align}
    Q = a_1 a_1^T - \tilde{a}_1 \tilde{a}_1,
\end{align}
resulting in the Hurwitz continuous-time stability relation (roots on stable left-half plane) of
\begin{equation}
\label{eq:stable_hermite}
    0 = \begin{bmatrix}
        0_{n \times 1} & H \\ 0 & 0_{1 \times n} 
    \end{bmatrix}  + \begin{bmatrix}
         0_{1 \times n}  & 0 \\ H &  0_{n \times 1}
    \end{bmatrix}.
\end{equation}
The unique solution to \eqref{eq:stable_hermite} may be discovered through the following forward substitution:
\begin{align}
    \forall j\in 2..n_a-1, i\in 1..n_a-1
    H_{i,j} = Q_{i+1, j} - H_{i+1, j-1}
\end{align}
\urg{Write the Hermite Matrix for continuous-time systems.
Is it
\begin{equation}
    0 = \begin{bmatrix}
        0_{n \times 1} & H \\ 0 & 0_{1 \times n} 
    \end{bmatrix}  + \begin{bmatrix}
         0_{1 \times n}  & 0 \\ H &  0_{n \times 1}
    \end{bmatrix}
\end{equation}

}

\subsection{Closed-Loop System Identification}

The Bode-plot data in $\dc$ for \eqref{eq:gain_base} was collected in open-loop. This extension involves the case where the unknown plant $G(z) = B(z^{-1})/(1+A(z^{-1}))$ is connected in feedback with a known dynamic compensator $C(z) = \tilde{B}(z^{-1})/(1+\tilde{A}(z^{-1})).$ The closed-loop transfer function of the plant $G(z)$ with a feedback controller $C(z)$ is

\begin{align}
G^{cl}(z) &= 
    \frac{B^{cl}(z^{-1})}{1+A^{cl}(z^{-1})}= \frac{G(z^{-1})}{1 + G(z^{-1}) C(z^{-1})} \label{eq:closed_loop} \\ 
    & = \frac{B(z^{-1}) (1+\tilde{A}(z^{-1}))}{(1+A(z^{-1}))(1+ \tilde{A}(z^{-1})) + B(z^{-1}) \tilde{B}(z^{-1})} \nonumber 
    \end{align}

The closed-loop optimization problem is
\begin{align}
    P^*_{cl} = \textstyle \inf_{a, b} \sum_{f=1}^{N_f} \abs{G_f^{cl} - G^{cl}(e^{j \omega_f})}^2. \label{eq:gain_closed_loop}
\end{align}

The following functions may be defined:
\begin{subequations}
\label{eq:poly_closed}
\begin{align}
    D_f^{cl}(a, b) &= (1+A(e^{-j \omega_f}))(1+ \tilde{A}(e^{-j \omega_f}))  \nonumber \\
    & \qquad + B(e^{-j \omega_f}) \tilde{B}(e^{-j \omega_f}) \\    
    p_f^{cl}(a, b) &= \abs{G_f D_f(a, b) - B(e^{-j \omega_f})(1 + \tilde{A}(e^{-j \omega_f}))}^2 \label{eq:poly_base_num_closed}\\
    q_f^{cl}(a) &= \abs{D_f(a, b)}^2,
\end{align}
\end{subequations}
% may be expressed as a sum of rational functions
% after requisite algebraic manipulations into
    % We can express \eqref{eq:closed_loop} at each frequency datapoint $f$ as a rational function of the plant parameters $(a, b)$ after requisite algebraic manipulations
    % \begin{align}
    %     G^{cl}_f = p^{cl}_f(a, b)/q^{cl}_f(a, b).
    % \end{align}
    % Problem \eqref{eq:gain_base} can therefore be expressed in the closed-loop case as 
to create the sum-of-rational-functions form for \eqref{eq:gain_closed_loop} as    
    \begin{align}
\label{eq:rational_closed}
    P^*_{cl} = \inf_{a, b} \textstyle \sum_{f=1}^{N_f} p_f^{cl}(a, b)/q_f^{cl}(a, b).
\end{align} 

Note that the denominator polynomial $q_f^{cl}$ in \eqref{eq:rational_closed} depends on $b$, due to the feedback with $C(z)$ in \eqref{eq:closed_loop}. The moment-\ac{SOS} \ac{LMI} derived from  a degree-$d$ truncation of \eqref{eq:rational_closed} will therefore not generally possess term sparsity \citep{wang2021tssos}.

If it is assumed that the closed-loop system $G^{cl}(z)$ is stable, then the Hermite stability constraint in $\mathcal{S}$ must be posed over the non-constant-coefficient vector of the closed-loop denominator in \eqref{eq:closed_loop} ($1+G(z^{-1}) C(z^{-1})$).



==> sections_extended/rational_sdp.tex <==
\section{Sum-of-Rational Semidefinite Program}

\label{sec:mom_sdp}

This section analyzes finite-degree moment-\ac{SOS} truncations to \eqref{eq:rational_meas_sparse}.

\subsection{LMI and Convergence}


A degree-$k$ truncation of \eqref{eq:rational_meas_sparse} with pseudomoment sequences $(y, y^f)$ for $(\mu, \nu^f)$ from \eqref{eq:sum_of_rational_mom_abscont} is
\begin{subequations}
\begin{align}
\label{eq:sum_of_rational_mom_abscont_sysid}
    p^*_k =& \inf_{y, y^f} \textstyle  \sum_{f=1}^L \mathbb{L}_{y^f}(p_f(a, b)) \\
    & y_\0 = 1 \\
    & \forall f \in 1, \ldots, N_f, (\alpha, \beta) \in \N^n_{2d} \nonumber \\
    &\qquad \mathbb{L}_{y^f}(a^\alpha b^\beta q_f(a))  =   \mathbb{L}_{y}(a^\alpha b^\beta) \label{eq:sum_of_rational_mom_abscont_marg} \\
    & \M_k[\K y], \forall f: \M_{k + 1 }[\K y^f] \succeq 0\label{eq:sum_of_rational_mom_abscont_mom}.
\end{align}
\end{subequations}

% It is required that $d\geq n$ and in order to pose Problem \eqref{eq:sum_of_rational_mom_abscont_sysid}.


\begin{cor}
    The sequence of objectives in \eqref{eq:sum_of_rational_mom_abscont} will satisfy $p^*_k \geq p^*_{k+1} \geq \ldots $ from \eqref{eq:gain_rat} under A1-A3 over $\K_0$.
\end{cor}
\begin{pf}
Monotonic increases in the cost functions will hold by raising the number of truncated moments considered in the infinite-dimensional matrix constraints \cite{lasserre2009moments}.
    % This convergence is established by  sufficiency of conditions from Theorem 2.2 of \cite{bugarin2016minimizing}. Even though we do not prove (or have) that $q_f(a) > 0$ over $\K$, 
\end{pf}

\begin{thm}
    The sequence of objectives in \eqref{eq:sum_of_rational_mom_abscont} will converge as $\lim_{k \rightarrow \infty} p^*_k = P^*$ under A1-A3 over $\K_s$.
\end{thm}
\begin{pf}
    All conditions of Theorem \ref{thm:bugarin_lmi} (Theorem 2.2 of \citep{bugarin2016minimizing}) are met (compactness condition, positivity of $q_f$ over $\K_s$), thus affirming convergence in degree.
\end{pf}

\subsection{Computational Complexity}

The computational complexity of solving a moment-\ac{SOS} \ac{LMI} of the form in \eqref{eq:moment_trunc} ($N$ variables, $k$-degree, single moment matix $\M_d[y]$ of size $\binom{N+k}{k}$) using an interior-point \ac{SDP} (up to $\epsilon$-accuracy) is $O(N^{6k})$ or $O(k^{4N})$ \citep{lasserre2009moments, miller2022data}.

Problem \eqref{eq:gain_rat} is an optimization problem posed over the $2n$ variables $(a, b)$. Table \ref{tab:mom_size} records the sizes and multiplicities of the matrix variables in \eqref{eq:sum_of_rational_mom_abscont_sysid} when the full monomial basis is used to describe constraints.

\begin{table}[h]
    \centering
    \caption{Size of \ac{PSD} matrix variables in \ac{LMI} \eqref{eq:sum_of_rational_mom_abscont_sysid}}
    \begin{tabular}{c c c c c}
    Measure & Matrix &  Size ($\K_0$) & Size ($\K_s$) & Multiplicity \\ \hline
        $\mu$ & $\M_d[\K y]$ & $\binom{n+d}{d}$ & $(n+1)\binom{n+k-1}{k-1}$& 1 \\
        $\nu_f$ & $\M_{k+1}[\K y^f]$ & $\binom{n + k+1}{k+1}$ & $(n+1)\binom{n+k}{k}$& $N_f$
    \end{tabular}
    \label{tab:mom_size}
\end{table}

The largest \ac{PSD} matrix for each measure over $\K_0$ is the moment matrix $(\M_k[y], \M_{k+1}[y^f])$. The largest \ac{PSD} block for $\K_s$ occurs in the stabilizing-\ac{PMI} constraint \eqref{eq:stable_pmi} with localizing matrix $(\M_d[\mathcal{S} y], \M_{k+1}[\mathcal{S} y^f])$

The computational scaling for fixed $n$ therefore grows exponentially in $k$ and linearly in $N_f$, according to the dominant \ac{PSD} blocks for $\nu_f$ of size $\binom{n+k+1}{k+1}$ ($\K_0$) or $(k+1)\binom{k+d}{d}$ ($\K_s$). By construction, the non-\ac{PMI} localizing matrix blocks (such as $\M_{d+1}[g_j(a, b) y^f] \succeq 0$ for a describing constraint polynomial $g_j(a, b)$ of $\K$) will have a smaller size than the moment block $\M_{k+1}[y^f]$.

Equation \eqref{eq:sum_of_rational_mom_abscont_marg} possesses an expoitable Term Sparsity in the sense of \citep{wang2021tssos}. The left-hand side of \eqref{eq:sum_of_rational_mom_abscont_marg} does not place any equality constraints on moments $y^f_{\alpha \beta}$ with $\sum_{i=1}^n \beta_i \in [n+1, n+2]$, given that $q_f(a)$ is independent of $b$. The these high-$b$-degree moments of $y^f$ purely act to ensure that $\M_{d+1}[\K y^f]$ is \ac{PSD}, and are not involved in the constraints nor the objective of \eqref{eq:sum_of_rational_mom_abscont}. The term sparsity method of \citep{wang2021tssos} can block-diagonalize the moment matrices $\M_{d+1}[\K y^f]$ to reduce dimensionality of the \ac{PSD} matrix constraints without introducing any conservatism (change in objective $p^*_k$ at degree $d$).

\subsection{Recovery of Optimal Plant}

% \begin{rmk}
    % A globally optimal set of plants $(a^*, b^*)$ can be extracted from the moment matrices $\M_d[\K y], \forall f: \M_{d + n }[\K y^f]$ if they are all rank-$r$ and have identical supports (Theorem 2.2 of \cite{bugarin2016minimizing}).
% \end{rmk}

% In practice, the rank and support points of all moment matrices might not be equal to $r$. 

Let us assume that \eqref{eq:sum_of_rational_mom_abscont_sysid} is solved at degree $d$ to produce an objective $p^*_d \leq P^*$ and moment matrix $\M_d[y]$

Further assume that the moment matrix $\M_d[y]$ satisfies \eqref{eq:flat_extension} with rank $r'$ and support points $\{(a^*_k, b^*_c)\}_{c=1}^{r'}$. If there exists a sufficiently small $\epsilon \geq 0$ such that  one of the support points $c$ satisfies $\textrm{MSE}_\dc(a^*_c, b^*_c) \in [p^*_k, p^*_k + \epsilon]$, then the point $(a^*_c, b^*_c)$ is approximately optimal. 

Other approximate extraction methods to generate candidate plants $(a, b)$ from the pseudo-moment matrix $\M_k[\K y]$ (even without satisfying the rank constraint \eqref{eq:flat_extension}) include \citep{garcia2021approximate, marx2021semi}. This condition is sufficient for recovery, but finite-degree bounds for when the rank constraint \eqref{eq:flat_extension} would be satisfied may not exist.


% \urg{How do we choose $\epsilon$? must be based on values of the MSE.}

% The nearly optimal extraction scheme 
% Practical values of $\epsilon$ could be in the range of $10^{-3}$, as compared to \ac{MSE} value 

% Nearly-optimal plants could be extracted from 


% \urg{The main theory}

% \urg{Finishing this after lunch}

==> sections_extended/report_summary.tex <==

This paper is an extended version of the report in \cite{abdalmoaty2023rationalsysid}.

==> sections_extended/summary.tex <==

This paper has the following structure: Section \ref{sec:preliminaries} introduces the notation used, reviews the moment-\ac{SOS} hierarchy of \acp{SDP}, and the sum-of-rational framework of \cite{bugarin2016minimizing}. Section \ref{sec:rational_sysid} casts the global optimization task in \eqref{eq:gain_base} as a real-valued sum-of-rational optimization problem. Section \ref{sec:mom_sdp} formulates finite-degree \ac{LMI} truncations of the sum-of-rational \acp{LP} and tabulates their \ac{SDP}-based computational complexity. Section \ref{sec:other_rational} adapts the sum-of-rational framework towards other experimental setups (e.g., continuous-time systems, closed-loop system identification). Section \ref{sec:outlier} incorporates outlier-rejection into system identification.
Section \ref{sec:examples} performs numerical examples and demonstrates the success of our method on global recovery, even while local-optimization based system identification methods return inaccurate systems. 
% Section \ref{sec:extensions} discusses extensions of this method, such as minimax estimators.
Section \ref{sec:conclusion} concludes the paper. 
Appendix \ref{app:strong_dual_lp} proves weak and strong duality properties between the sum-of-rational \acp{LP}. 
% Appendix \ref{app:fractional} comments on Hermite-based stability constraints for commensurate fractional-order linear systems.
% \urg{Fill in the paper structure}
% Section \ref{sec:preliminaries} will review preliminaries such as notation, notions of stability for linear systems, and \ac{SOS} proofs of polynomial nonnegativity. Section \ref{sec:full_method} will present 
% The paper is concluded in Section \ref{sec:conclusion}.
